Distilling Stereo Networks for Performant and Efficient Leaner Networks

Knowledge distillation has been quite popular in vision for tasks like classification and segmentation however not much work has been done for distilling state-of-the-art stereo matching methods despite their range of applications. One of the reasons for its lack of use in stereo matching networks is due to the inherent complexity of these networks, where a typical network is composed of multiple two- and three-dimensional modules. In this work, we systematically combine the insights from state-of-the-art stereo methods with general knowledge-distillation techniques to develop a joint framework for stereo networks distillation with competitive results and faster inference. Moreover, we show, via a detailed empirical analysis, that distilling knowledge from the stereo network requires careful design of the complete distillation pipeline starting from backbone to the right selection of distillation points and corresponding loss functions. This results in the student networks that are not only leaner and faster but give excellent performance . For instance, our student network while performing better than the performance oriented methods like PSMNet [1], CFNet [2], and LEAStereo [3]) on benchmark SceneFlow dataset, is 8x, 5x, and 8x faster respectively. Furthermore, compared to speed oriented methods having inference time less than 100ms, our student networks perform better than all the tested methods. In addition, our student network also shows better generalization capabilities when tested on unseen datasets like ETH3D and Middlebury.

==> architecture-blocks.tex <==
\begin{figure}[htb!]
     \centering
     \begin{subfigure}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=0.5\columnwidth]{./images/backbone-B1.pdf}
         \caption{B1 block}
         \label{fig:b1}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[b]{0.45\columnwidth}
%         \centering
         \includegraphics[width=0.75\columnwidth]{./images/backbone-B2.pdf}
         \caption{B2 block}
         \label{fig:b2}
     \end{subfigure}
%     \hfill
        \caption{Design of B1 and B2 blocks in feature extraction module.}
        \label{fig:blocks}
\end{figure}

==> results/ablation-study.tex <==
\begin{table}[]
	\centering
		\renewcommand{\arraystretch}{1.2}
	\begin{adjustbox}{width=\columnwidth}
		\npdecimalsign{.}
		\nprounddigits{2}
		\begin{tabular}{l|c|c|c|c|c|c|n{2}{3}} %|n{2}{3}|n{2}{2}|n{2}{2}|n{2}{2}|n{2}{2}|
			\hline
			\makecell{Loss\\Function} & {\spw} & {\cv} & {\fe} & {\ca} & {\stpw} & \makecell{\cv+\\Attention} & {EPE($px$)}\\ \hline
			\hline
			smoothL1 & \checkmark &  &   &  &  &   & 0.79  \\
			LogL1 & \checkmark &  &   &  &  &    & 0.76  \\
			\hline
			
			MSE & \checkmark & \checkmark  &   &  &  & &  0.75 \\					
			KLD & \checkmark & \checkmark  &   &  &  &   & 0.72 \\
			Cosine & \checkmark & \checkmark  &   &  &  &   & 0.71 \\			
			LogL1 & \checkmark & \checkmark  &   &  &  &   & 0.77  \\		
			\hline
			
			MSE & \checkmark & \checkmark  & \checkmark &  &  &   & 0.74  \\		
			KLD & \checkmark & \checkmark  & \checkmark &  &  &   & 0.73  \\		
			Cosine & \checkmark & \checkmark  & \checkmark &  &  &  &  0.71  \\		
			LogL1 & \checkmark & \checkmark  & \checkmark &  &  &   & 0.74  \\	
			\hline
			
			MSE & \checkmark & \checkmark  & \checkmark & \checkmark &  &  &  0.71    \\		
			KLD & \checkmark & \checkmark  & \checkmark & \checkmark &  &   & 0.65  \\		
			Cosine & \checkmark & \checkmark  & \checkmark & \checkmark &  &   & 0.66    \\		
			LogL1 & \checkmark & \checkmark  & \checkmark & \checkmark &  &   & 0.69  \\	
			\hline
			
			LogL1 & \checkmark & \checkmark  & \checkmark & \checkmark & \checkmark &   & 0.65 \\	
			smoothL1 & \checkmark & \checkmark  & \checkmark & \checkmark & \checkmark &   & 0.62    \\	
			\hline
			
			Cosine & \checkmark & \checkmark  & \checkmark & \checkmark & \checkmark & \checkmark  & 0.55   \\
				
			\hline
		\end{tabular}
	\end{adjustbox}
	\caption{Results of ablation study of distillation points and losses on \sf \cite{mayer_large_2016} dataset.}
	\label{table:ablation-study}
\end{table}


%%\begin{table*}[]
%	\centering
%	%	\begin{adjustbox}{width=\columnwidth}
%	\npdecimalsign{.}
%	\nprounddigits{2}
%	\begin{tabular}{|r|c|c|c|c|c|c|n{2}{3}|n{2}{3}|n{2}{3}|n{2}{3}|n{2}{3}|} %|n{2}{3}|n{2}{2}|n{2}{2}|n{2}{2}|n{2}{2}|
%		\hline
%		\makecell{Loss\\Function} & {spw} & \makecell{Cost\\Aggregation} & \makecell{Cost\\Volume} & \makecell{Early\\Features} & {stpw} & \makecell{Attention in \\ Cost Volume} & {EPE ($px$)} & {D1 ($\%$)}  & {px-3 ($\%$)}  & {px-2 ($\%$)} & {px-1 ($\%$)}\\ \hline
%		\hline
%		smoothL1 & \checkmark &  &   &  &  &   & 0.8807 & 3.188 & 3.799 & 5.115 & 9.145  \\
%		LogL1 & \checkmark &  &   &  &  &    & 0.8221 & 2.851 & 3.345 & 4.219 & 6.565  \\
%		\hline
%		
%		MSE & \checkmark & \checkmark  &   &  &  & &  0.8308 & 2.842 & 3.34 & 4.267 & 6.833   \\					
%		KLD & \checkmark & \checkmark  &   &  &  &   & 0.8023 & 3.321 & 3.897 & 4.995 & 7.863 \\
%		Cosine & \checkmark & \checkmark  &   &  &  &   & 0.8254 & 2.867 & 3.38 & 4.314 & 6.843   \\			
%		LogL1 & \checkmark & \checkmark  &   &  &  &   & 0. & 0. & 0. & 0. & 0.    \\		
%		\hline
%		
%		MSE & \checkmark & \checkmark  & \checkmark &  &  &   & 0. & 0. & 0. & 0. & 0.    \\		
%		KLD & \checkmark & \checkmark  & \checkmark &  &  &   & 0. & 0. & 0. & 0. & 0.    \\		
%		Cosine & \checkmark & \checkmark  & \checkmark &  &  &  &  0. & 0. & 0. & 0. & 0.    \\		
%		LogL1 & \checkmark & \checkmark  & \checkmark &  &  &   & 0. & 0. & 0. & 0. & 0.    \\	
%		\hline
%		
%		MSE & \checkmark & \checkmark  & \checkmark & \checkmark &  &  &  0.8054 & 2.795 & 3.284 & 4.152 & 6.498    \\		
%		KLD & \checkmark & \checkmark  & \checkmark & \checkmark &  &   & 0. & 0. & 0. & 0. & 0.    \\		
%		Cosine & \checkmark & \checkmark  & \checkmark & \checkmark &  &   & 0.7576 & 2.634 & 3.122 & 3.994 & 6.372    \\		
%		LogL1 & \checkmark & \checkmark  & \checkmark & \checkmark &  &   & 0. & 0. & 0. & 0. & 0.    \\	
%		\hline
%		
%		LogL1 & \checkmark & \checkmark  & \checkmark & \checkmark & \checkmark &   & 0.7538 & 2.552 & 3.04 & 3.902 & 6.319   \\	
%		smoothL1 & \checkmark & \checkmark  & \checkmark & \checkmark & \checkmark &   & 0.7186 & 2.664 & 3.164 & 4.078 & 6.562    \\	
%		\hline
%		
%		Consine & \checkmark & \checkmark  & \checkmark & \checkmark & \checkmark & \checkmark  & 0.6419 & 2.284 & 2.767 & 3.621 & 5.974   \\
%		
%		\hline
%	\end{tabular}
%	%	\end{adjustbox}
%	\caption{Different variants/cadidates of the student network. For all metrics, lower is better.}
%	\label{table:ablation-study}
%\end{table*}

==> results/dist-affect-attention.tex <==
\begin{table}[]
	\centering
	\def\arraystretch{1.5}
	\begin{adjustbox}{width=\columnwidth}
		\npdecimalsign{.}
		\nprounddigits{2}
		\begin{tabular}{c|n{2}{3}|n{2}{3}|n{2}{3}|n{2}{3}|n{2}{3}} %|n{2}{3}|n{2}{2}|n{2}{2}|n{2}{2}|n{2}{2}|
			\hline
			\makecell{Distillation\\in Student Network}  & {EPE($px$)} & {D1($\%$)}  & {\dpix($\%$)} & {\tpix($\%$)} & {\opix($\%$)}\\ \hline
			\hline
			\xmark & 0.7078 &  2.448 &  2.918 & 3.707 & 5.822 \\
			\checkmark &  0.6419 & 2.284 & 2.767 & 3.621 & 5.974 \\

			\hline
		\end{tabular}
	\end{adjustbox}
	\caption{Effect of \kd on the attention based student network.}
	\label{table:dist-affect-attention}
\end{table}

==> results/generalization.tex <==
%\begin{table}[tbh!]
%
%		\centering
%	\begin{adjustbox}{width=\columnwidth}
%		\begin{tabular}{c|c|c|c|c|c|c} %|n{2}{3}|n{2}{2}|n{2}{2}|n{2}{2}|n{2}{2}|
%			\hline
%			Dataset  & Metric & CRL\cite{pang2017cascade}  & PSMNet\cite{chang_pyramid_2018} & HITNet\cite{tankovich2021hitnet} &  EdgeStereo\cite{song2020edgestereo} & Ours\\ \hline
%			%			Baseline \cite{guo_group-wise_2019} & 6.52 & 246.27 & 0.8661 & 3.195 & 3.783 \\
%			\hline
%			\multirow{3}{*}{\kitti 2012\cite{geiger2012we}} & EPE & 1.38 & 5.54 & 1.06 & 1.96 & 1.46 \\
%			& \dpix  & 9.07  & 27.33 & 6.44 & 12.27 & 8.20 \\
%			& {D1($\%$)} & - & - & - & - & 7.76 \\ 
%			\hline
%			\multirow{3}{*}{\kittif\cite{menze_object_2015}} & EPE & 1.35 & 6.44 & 1.36 & 2.06 & 1.73 \\
%			& \dpix &  8.88 & 29.86 & 6.49  & 12.46 & 8.283 \\
%			& {D1($\%$)} & - & - & - & - & 8.06  \\ 
%			\hline
%		\end{tabular}
%	\end{adjustbox}
%	\caption{Quantifying the generalization capability of student network. These models are trained on \sf dataset are tested on \kitti 2012 and \kittif datasets, respectively.}
%	\label{table:generalization}
%\end{table}
%


\begin{figure*}[thb!]
	\vspace*{-10pt}
	\centering
	\begin{tabular}{ccc}
		%		& \multicolumn{2}{c}{Example 1} &  \\
		& \textit{\kitti 2012 Examples} &   \\
		
		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000039_10_2new.png} &	\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000039_10_0.png} &		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000039_10_1.png} \\
		
		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000059_10_2new.png} &	\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000059_10_0.png} &		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000059_10_1.png} \\		
		
		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000139_10_2new.png} &	\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000139_10_0.png} &		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000139_10_1.png} \\
		
		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000119_10_2new.png} &	\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000119_10_0.png} &		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000119_10_1.png} \\
		
		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000159_10_2new.png} &	\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000159_10_0.png} &		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000159_10_1.png} \\
%		Left Image & Predicted Disparity Map & Error Map \\ 
	\end{tabular}
	
	\begin{tabular}{ccc}
		%		& \multicolumn{2}{c}{Example 1} &  \\
		& \textit{\mb Examples}&   \\
		\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/input/rahim_data_MiddEval3_trainingH_Adirondack_im0.png} &	\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/pred/rahim_data_MiddEval3_trainingH_Adirondack_im0.png} &		\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/pred-errormap/rahim_data_MiddEval3_trainingH_Adirondack_im0.png} \\
		 
%		\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/input/rahim_data_MiddEval3_trainingH_MotorcycleE_im0.png} &	\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/pred/rahim_data_MiddEval3_trainingH_MotorcycleE_im0.png} &		\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/pred-errormap/rahim_data_MiddEval3_trainingH_MotorcycleE_im0.png} \\		
		
		\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/input/rahim_data_MiddEval3_trainingH_PlaytableP_im0.png} &	\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/pred/rahim_data_MiddEval3_trainingH_PlaytableP_im0.png} &		\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/pred-errormap/rahim_data_MiddEval3_trainingH_PlaytableP_im0.png} \\
		
		\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/input/rahim_data_MiddEval3_trainingH_Recycle_im0.png} &	\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/pred/rahim_data_MiddEval3_trainingH_Recycle_im0.png} &		\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/pred-errormap/rahim_data_MiddEval3_trainingH_Recycle_im0.png} \\
		
		Left Image & Predicted Disparity Map & Error Map  \\
	\end{tabular}
	\caption{Generalization results of \dsnet, trained on \sf dataset and evaluated on \kitti and \mb datasets.}
	\label{fig:generalization-quality}
\end{figure*}

%\begin{figure*}[thb!]
%	\vspace*{-10pt}
%	\centering
%	\begin{tabular}{ccc}
%		%		& \multicolumn{2}{c}{Example 1} &  \\
%		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000039_10_2new.png} &	\includegraphics[width=0.33\linewidth]{./results/images/kitti-generalization/000039_10_0.png} &		\includegraphics[width=0.33\linewidth]{./results/images/kitti-generalization/000039_10_1.png} \\
%		
%		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000059_10_2new.png} &	\includegraphics[width=0.33\linewidth]{./results/images/kitti-generalization/000059_10_0.png} &		\includegraphics[width=0.33\linewidth]{./results/images/kitti-generalization/000059_10_1.png} \\		
%		
%		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000139_10_2new.png} &	\includegraphics[width=0.33\linewidth]{./results/images/kitti-generalization/000139_10_0.png} &		\includegraphics[width=0.33\linewidth]{./results/images/kitti-generalization/000139_10_1.png} \\
%		
%		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000119_10_2new.png} &	\includegraphics[width=0.33\linewidth]{./results/images/kitti-generalization/000119_10_0.png} &		\includegraphics[width=0.33\linewidth]{./results/images/kitti-generalization/000119_10_1.png} \\
%		
%		\includegraphics[width=0.32\linewidth]{./results/images/kitti-generalization/000159_10_2new.png} &	\includegraphics[width=0.33\linewidth]{./results/images/kitti-generalization/000159_10_0.png} &		\includegraphics[width=0.33\linewidth]{./results/images/kitti-generalization/000159_10_1.png} \\
%		Left Image & Predicted Disparity Map & Error Map  \\
%	\end{tabular}
%	\caption{Output of student network trained on synthetic \sf dataset and being evaluated on real-world \kitti 2012.}
%	\label{fig:generalization-quality}
%\end{figure*}
%
%\begin{figure*}[thb!]
%	\vspace*{-10pt}
%	\centering
%	\begin{tabular}{ccc}
%		%		& \multicolumn{2}{c}{Example 1} &  \\
%		\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/input/rahim_data_MiddEval3_trainingH_Adirondack_im0.png} &	\includegraphics[width=0.33\linewidth]{./results/images/mb-generalization/pred/rahim_data_MiddEval3_trainingH_Adirondack_im0.png} &		\includegraphics[width=0.33\linewidth]{./results/images/mb-generalization/pred-errormap/rahim_data_MiddEval3_trainingH_Adirondack_im0.png} \\
%		
%		\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/input/rahim_data_MiddEval3_trainingH_MotorcycleE_im0.png} &	\includegraphics[width=0.33\linewidth]{./results/images/mb-generalization/pred/rahim_data_MiddEval3_trainingH_MotorcycleE_im0.png} &		\includegraphics[width=0.33\linewidth]{./results/images/mb-generalization/pred-errormap/rahim_data_MiddEval3_trainingH_MotorcycleE_im0.png} \\		
%		
%		\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/input/rahim_data_MiddEval3_trainingH_PlaytableP_im0.png} &	\includegraphics[width=0.33\linewidth]{./results/images/mb-generalization/pred/rahim_data_MiddEval3_trainingH_PlaytableP_im0.png} &		\includegraphics[width=0.33\linewidth]{./results/images/mb-generalization/pred-errormap/rahim_data_MiddEval3_trainingH_PlaytableP_im0.png} \\
%		
%		\includegraphics[width=0.32\linewidth]{./results/images/mb-generalization/input/rahim_data_MiddEval3_trainingH_Recycle_im0.png} &	\includegraphics[width=0.33\linewidth]{./results/images/mb-generalization/pred/rahim_data_MiddEval3_trainingH_Recycle_im0.png} &		\includegraphics[width=0.33\linewidth]{./results/images/mb-generalization/pred-errormap/rahim_data_MiddEval3_trainingH_Recycle_im0.png} \\
%		
%		Left Image & Predicted Disparity Map & Error Map  \\
%	\end{tabular}
%	\caption{Generalization results of \dsnet, trained on \sf dataset, evaluated on \mb dataset.}
%	\label{fig:generalization-quality-mb}
%\end{figure*}

==> results/kitti15_benchmark_quality.tex <==
\begin{figure*}
%	\footnotesize		
	\begin{adjustbox}{width=\linewidth}
	\begin{tabular}{m{0.2em}ccc}
		 {\rotatebox[origin=c]{90}{\textit{Left Image}}}	& \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/input-gt/left-images/000002_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/input-gt/left-images/000019_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/input-gt/left-images/000005_10.png}\\
% 		& Left Images & \\
		
		\multirow{2}{*}{ \rotatebox{90}{\textit{GANet\cite{zhang_ga-net:_2019}}}}&
		\includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/ganet/pred/000002_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/ganet/pred/000019_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/ganet/pred/000005_10.png} \\
		
		&\includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/ganet/pred-errormap/000002_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/ganet/pred-errormap/000019_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/ganet/pred-errormap/000005_10.png} \\
%		& GANet\cite{zhang_ga-net:_2019} & \\
		
		\multirow{2}{*}{ \rotatebox{90}{\textit{PSMNet\cite{chang_pyramid_2018}}}}&
		\includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/psmnet/pred/000002_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/psmnet/pred/000019_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/psmnet/pred/000005_10.png} \\
		
		&\includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/psmnet/pred-errormap/000002_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/psmnet/pred-errormap/000019_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/psmnet/pred-errormap/000005_10.png} \\
%		& PSMNet\cite{chang_pyramid_2018} & \\
		
		\multirow{2}{*}{\rotatebox{90}{\textit{GwcNet-g\cite{guo_group-wise_2019}}}}&
		\includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/gwcnet/pred/000002_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/gwcnet/pred/000019_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/gwcnet/pred/000005_10.png} \\
		
		&\includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/gwcnet/pred-errormap/000002_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/gwcnet/pred-errormap/000019_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/gwcnet/pred-errormap/000005_10.png} \\
%		& GwcNet-g\cite{guo_group-wise_2019} & \\
		
		\multirow{2}{*}{\rotatebox{90}{\textit{ACVNet\cite{xu2022acvnet}}}}&
		\includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/acvnet/pred/000002_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/acvnet/pred/000019_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/acvnet/pred/000005_10.png} \\
		
		&\includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/acvnet/pred-errormap/000002_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/acvnet/pred-errormap/000019_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/acvnet/pred-errormap/000005_10.png} \\
%		& ACVNet\cite{xu2022acvnet} & \\
		
		
		\multirow{2}{*}{\rotatebox{90}{\textit{\dsnet}}}&
		\includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/our-distill/pred/000002_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/our-distill/pred/000019_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/our-distill/pred/000005_10.png} \\
		
		&\includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/our-distill/pred-errormap/000002_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/our-distill/pred-errormap/000019_10.png} & \includegraphics[width=0.33\linewidth]{./results/images/kitti-benchmark/our-distill/pred-errormap/000005_10.png} \\
%		&  Ours & \\
	\end{tabular}
	\end{adjustbox}
	\caption{Results (disparity images together with error maps)  of running student network on \kittif benchmark dataset -- these images are downloaded from the benchmark website. Warmer colors in error maps denote larger error values. }
	\label{fig:kitti15-benchmark-quality}
	
\end{figure*}


%\begin{figure*}[htpb]
%	\captionsetup[subfiguOurre]{labelformat=empty}
%	\centering
%	\begin{center}
%		\begin{minipage}[c]{0.01\textwidth}
%			\begin{turn}{90}\footnotesize{}\end{turn}			
%		\end{minipage}
%		\begin{minipage}[c]{0.985\textwidth}
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000001_10.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000005_10.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000009_10.png}
%			\end{subfigure}
%		\end{minipage}
%		\\Our
%		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		\begin{minipage}[c]{0.01\textwidth}
%			\begin{turn}{90}\footnotesize{GCNet \cite{kendall_end--end_2017}}\end{turn}			
%		\end{minipage}
%		\begin{minipage}[c]{0.985\textwidth}
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000001_10_1__GC.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000005_10_1__GC.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000009_10_1__GC.png}
%			\end{subfigure}
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000001_10_2__GC.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000005_10_2__GC.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000009_10_2__GC.png}
%			\end{subfigure}
%		\end{minipage}
%		\\
%		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		\begin{minipage}[c]{0.01\textwidth}
%			\begin{turn}{90}\footnotesize{PSMNet \cite{chang_pyramid_2018}}\end{turn}			
%		\end{minipage}
%		\begin{minipage}[c]{0.985\textwidth}
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000001_10_1__PSMNet.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000005_10_1__PSMNet.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000009_10_1__PSMNet.png}
%			\end{subfigure}
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000001_10_2__PSMNet.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000005_10_2__PSMNet.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000009_10_2__PSMNet.png}
%			\end{subfigure}
%		\end{minipage}
%		\\
%		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		\begin{minipage}[c]{0.01\textwidth}
%			\begin{turn}{90}\footnotesize{GwcNet-g \cite{guo_group-wise_2019}}\end{turn}			
%		\end{minipage}
%		\begin{minipage}[c]{0.985\textwidth}
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000001_10_1__GWCNET_G.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000005_10_1__GWCNET_G.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000009_10_1__GWCNET_G.png}
%			\end{subfigure}
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000001_10_2__GWCNET_G.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000005_10_2__GWCNET_G.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000009_10_2__GWCNET_G.png}
%			\end{subfigure}
%		\end{minipage}
%		\\
%		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		\begin{minipage}[c]{0.01\textwidth}
%			\begin{turn}{90}\footnotesize{ACVNet\cite{xu2022acvnet}}\end{turn}			
%		\end{minipage}
%		\begin{minipage}[c]{0.985\textwidth}
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000001_10_1__2D.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000005_10_1__2D.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000009_10_1__2D.png}
%			\end{subfigure}
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000001_10_2__2D.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000005_10_2__2D.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000009_10_2__2D.png}
%			\end{subfigure}
%		\end{minipage}
%		\\
%		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		\begin{minipage}[c]{0.01\textwidth}
%			\begin{turn}{90}\footnotesize{Our}\end{turn}			
%		\end{minipage}
%		\begin{minipage}[c]{0.985\textwidth}
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images//000001_10_1__3D.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000005_10_1__3D.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000009_10_1__3D.png}
%			\end{subfigure}
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images//000001_10_2__3D.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000005_10_2__3D.png}
%			\end{subfigure}
%			\hspace{-0.5\baselineskip}
%			\hfill
%			\begin{subfigure}[c]{0.33\linewidth}
%				\includegraphics[width=0.9\linewidth]{images/000009_10_2__3D.png}
%			\end{subfigure}
%		\end{minipage}
%		\\
%		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		\vspace{-0.2cm}
%		\caption{Qualitative performance (disparity images together with error maps) from KITTI 2015 benchmark. Warmer colors in error maps denote larger values.}
%		\vspace{-0.3cm}
%		\label{fig:KittiBenchmark}
%	\end{center}
%\end{figure*}

==> results/kitti15_val.tex <==
\begin{table}[tbp]
	\centering
	\begin{adjustbox}{width=\columnwidth}
		\begin{tabular}{l|ccc|cc}
			\hline				
			{Method} & {EPE($px$)} & {D1(\%)} & {px-3(\%)} & {MACs($G$)} & {Params($M$)} \\	\hline			
			\hline				
			PSMNet\cite{chang_pyramid_2018} & 0.88 & 2.00 & 2.10 & 256.66 & 5.22 \\
			GA-Net-deep\cite{zhang_ga-net:_2019} & 0.63 & 1.61 & 1.67 & 670.25 & 6.58 \\
			GA-Net-11\cite{zhang_ga-net:_2019}  & 0.67 & 1.92 & 2.01 & 383.42 & {4.48} \\
			GwcNet-gc\cite{guo_group-wise_2019} & 0.63 & 1.55 & 1.60 & 260.49 & 6.82 \\
			GwcNet-g\cite{guo_group-wise_2019}  & {0.62} & {1.49} & {1.53} & 246.27 & 6.43 \\
			MobileStereoNet\cite{shamsafar2022mobilestereonet}      & 0.66 & 1.59 & 1.69 & 153.14 & {1.77}\\	
			\hline
			Ours  & 0.62 & 1.59 & 1.76  & 91.33 & 1.86 \\			
			\hline				
		\end{tabular}
	\end{adjustbox}

	\caption{Comparison of competing methods on the \kittif validation set.}
	\label{table:kitti15-val}
\end{table}

==> results/memorytime.tex <==
\begin{table}[!htb]
	\begin{center}
		\begin{adjustbox}{width=\columnwidth}
			%		\footnotesize
			\begin{tabular}{c|r|r|c|r|r}
				\hline				
				{Method} & \makecell{Model\\Size(MB)} & \makecell{More \\ Size} & \makecell{Avg. Inference \\ time(msec)} & \makecell{More \\ time} & {MACs($G$)} \\				
				\hline
				\hline
				PSMNet\cite{chang_pyramid_2018}  & 21.12 & 2.8$\times$ & 619 & 7.7$\times$ & 256.66 \\
				GA-Net-deep\cite{zhang_ga-net:_2019}  & 26.45  & 3.5$\times$ & 3580 & 44.8$\times$  & 670.25 \\
				GA-Net-11\cite{zhang_ga-net:_2019}  & 18.00  & 2.4$\times$ & 2362 & 29.5$\times$  & 383.42 \\			
				GwcNet-g\cite{guo_group-wise_2019}  & 26.32  & 3.5$\times$ & 240 & 3$\times$  & 246.27 \\
				MobileStereoNet \cite{shamsafar2022mobilestereonet} & 10.03 &  1.3$ \times $ & 1500 & 18.6 $ \times $ & 153.14\\
				CFNet\cite{shen2021cfnet}  & 92.60  & 12.2$\times$ & 483 & 6.0$\times$  & 177.50 \\
				LEAStereo\cite{cheng2020hierarchical}  & 7.61  & 1.0$\times$ & 945 &11.8$\times$  & 156.50 \\
				ACVNet\cite{xu2022acvnet}   & 25.17  & 3.3$\times$ & 302 & 3.8$\times$  & 240.05 \\
				\hline
				Ours   & 7.56 & - & 80 & -  & 91.33  \\
				\hline				
			\end{tabular}
		\end{adjustbox}	
	\end{center}
	\vspace*{-0.5cm}
	\caption{Memory and inference time comparison of different methods on an NVIDIA GeForce RTX 2080 Ti with image size of $ 512 \times 960 $. }
	\label{table:memorytime}
	\vspace*{-0.6cm}
\end{table}


==> results/sf-quality.tex <==
\begin{figure*}[t]
	\centering
	\begin{adjustbox}{width=\linewidth}
	\begin{tabular}{m{0.5em}cccc}
		\multirow{2}{*}{ \rotatebox{90}{\textit{Example 1}}}&
		\includegraphics[width=0.23\linewidth]{./results/images/sceneflow/input-gt/left-images/A_0117_left_0006.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/gwcnet/pred-errormap/A_0117_left_0006.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/acvnet/pred-errormap/A_0117_left_0006.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/our-distill/pred-errormap/A_0117_left_0006.png} 
		\\
		&\includegraphics[width=0.23\linewidth]{./results/images/sceneflow/input-gt/GT-disparities/A_0117_left_0006.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/gwcnet/pred/A_0117_left_0006.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/acvnet/pred/A_0117_left_0006.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/our-distill/pred/A_0117_left_0006.png}
		\\
		
		\multirow{2}{*}{ \rotatebox{90}{\textit{Example 2}}}&
		\includegraphics[width=0.23\linewidth]{./results/images/sceneflow/input-gt/left-images/B_0023_left_0015.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/gwcnet/pred-errormap/B_0023_left_0015.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/acvnet/pred-errormap/B_0023_left_0015.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/our-distill/pred-errormap/B_0023_left_0015.png} 
		\\
		&\includegraphics[width=0.23\linewidth]{./results/images/sceneflow/input-gt/GT-disparities/B_0023_left_0015.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/gwcnet/pred/B_0023_left_0015.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/acvnet/pred/B_0023_left_0015.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/our-distill/pred/B_0023_left_0015.png}
		\\
		
		\multirow{2}{*}{ \rotatebox{90}{\textit{Example 3}}}&
		\includegraphics[width=0.23\linewidth]{./results/images/sceneflow/input-gt/left-images/A_0000_left_0006.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/gwcnet/pred-errormap/A_0000_left_0006.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/acvnet/pred-errormap/A_0000_left_0006.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/our-distill/pred-errormap/A_0000_left_0006.png} 
		\\
		&\includegraphics[width=0.23\linewidth]{./results/images/sceneflow/input-gt/GT-disparities/A_0000_left_0006.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/gwcnet/pred/A_0000_left_0006.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/acvnet/pred/A_0000_left_0006.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/our-distill/pred/A_0000_left_0006.png}
		\\
%		& \multicolumn{2}{c}{Example 3} &  \\
%		\includegraphics[width=0.23\linewidth]{./results/images/sceneflow/input-gt/left-images/A_0108_left_0010.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/gwcnet/pred-errormap/A_0108_left_0010.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/acvnet/pred-errormap/A_0108_left_0010.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/our/pred-errormap/A_0108_left_0010.png} 
%		\\
%		\includegraphics[width=0.23\linewidth]{./results/images/sceneflow/input-gt/GT-disparities/A_0108_left_0010.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/gwcnet/pred/A_0108_left_0010.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/acvnet/pred/A_0108_left_0010.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/our/pred/A_0108_left_0010.png}
%		\\
%		& \multicolumn{2}{c}{Example 4} &  \\
%		\includegraphics[width=0.23\linewidth]{./results/images/sceneflow/input-gt/left-images/B_0032_left_0015.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/gwcnet/pred-errormap/B_0032_left_0015.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/acvnet/pred-errormap/B_0032_left_0015.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/our/pred-errormap/B_0032_left_0015.png} 
%		\\
%		\includegraphics[width=0.23\linewidth]{./results/images/sceneflow/input-gt/GT-disparities/B_0032_left_0015.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/gwcnet/pred/B_0032_left_0015.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/acvnet/pred/B_0032_left_0015.png} &	\includegraphics[width=0.24\linewidth]{./results/images/sceneflow/our/pred/B_0032_left_0015.png}
%		\\
		&Left Image / GT & GwcNet-g\cite{guo_group-wise_2019} & ACVNet\cite{xu2022acvnet} & Ours  \\
	\end{tabular}
	\end{adjustbox}
	\caption{Qualitative results on SceneFlow test images. Here the first, third and fifth rows represent the left input images and error maps \wrt ground truth (GT). Seocnd, third and last rows show GT and predicted disparity maps. In error maps, darker red means high disparity errors and as the color gets more blue (darker blue) it represents lower disparity errors.}
	\label{fig:sf-quality}
\end{figure*}




==> results/teacher-networks.tex <==

\begin{table}[]
	\centering
	\def\arraystretch{1.5}
	\begin{adjustbox}{width=\columnwidth}
		\npdecimalsign{.}
		\nprounddigits{2}
		\begin{tabular}{l|n{2}{3}|n{2}{3}|n{2}{3}|n{2}{3}|n{2}{3}} %|n{2}{3}|n{2}{2}|n{2}{2}|n{2}{2}|n{2}{2}|
			\hline
			\makecell{Teacher\\Network}  & {EPE($px$)} & {D1($\%$)}  & {\dpix($\%$)} & {\tpix($\%$)} & {\opix($\%$)}\\ \hline
%			Baseline \cite{guo_group-wise_2019} & 6.52 & 246.27 & 0.8661 & 3.195 & 3.783 \\
			\hline
			\lacnet \cite{liu2022local} & 0.9831 & 4.12 & 4.736 & 6.085 & 9.43 \\
			\gwcnet \cite{guo_group-wise_2019} & 0.817 &  3.207 & 3.779 & 4.903 & 7.948 \\
			\acvnet \cite{xu2022acvnet} & 0.6419 & 2.284 & 2.767 & 3.621 & 5.974 \\
			
			\hline
		\end{tabular}
	\end{adjustbox}
	\caption{Effect of using different teacher networks for the training of the student network.}
	\label{table:teacher-networks}
\end{table}
